deepMiRGene: Deep Neural Network based Precursor microRNA Prediction

Since microRNAs (miRNAs) play a crucial role in post-transcriptional gene regulation, miRNA identification is one of the most essential problems in computational biology. miRNAs are usually short in length ranging between 20 and 23 base pairs. It is thus often difficult to distinguish miRNA-encoding sequences from other non-coding RNAs and pseudo miRNAs that have a similar length, and most previous studies have recommended using precursor miRNAs instead of mature miRNAs for robust detection. A great number of conventional machine-learning-based classification methods have been proposed, but they often have the serious disadvantage of requiring manual feature engineering, and their performance is limited as well. In this paper, we propose a novel miRNA precursor prediction algorithm, deepMiRGene, based on recurrent neural networks, specifically long short-term memory networks. deepMiRGene automatically learns suitable features from the data themselves without manual feature engineering and constructs a model that can successfully reflect structural characteristics of precursor miRNAs. For the performance evaluation of our approach, we have employed several widely used evaluation metrics on three recent benchmark datasets and verified that deepMiRGene delivered comparable performance among the current state-of-the-art tools.

==> acknowledgements.tex <==
Acknowledgements!!

 
\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
probably should) include acknowledgements. In this case, please
place such acknowledgements in an unnumbered section at the
end of the paper. Typically, this will include thanks to reviewers
who gave useful comments, to colleagues who contributed to the ideas, 
and to funding agencies and corporate sponsors that provided financial 
support.  


==> algorithm.tex <==
\makeatletter
\newcounter{ALC@tempcntr}% Temporary counter for storage
\newcommand{\LCOMMENT}[1]{%
    \setcounter{ALC@tempcntr}{\arabic{ALC@rem}}% Store old counter
    \setcounter{ALC@rem}{1}% To avoid printing line number
    \item {\(\triangleright\) #1}% Display comment + does not increment list item counter
    \setcounter{ALC@rem}{\arabic{ALC@tempcntr}}% Restore old counter
}%
\newcommand{\LCOMMENTR}[1]{%
    \setcounter{ALC@tempcntr}{\arabic{ALC@rem}}% Store old counter
    \setcounter{ALC@rem}{1}% To avoid printing line number
    \item {#1}% Display comment + does not increment list item counter
    \setcounter{ALC@rem}{\arabic{ALC@tempcntr}}% Restore old counter
}%
\newcommand\NoDo{\renewcommand\algorithmicdo{}}
\newcommand\ReDo{\renewcommand\algorithmicdo{\textbf{do}}}
\newcommand\NoThen{\renewcommand\algorithmicthen{}}
\newcommand\ReThen{\renewcommand\algorithmicthen{\textbf{then}}}
\def\sss{\scriptstyle}
\makeatother



\begin{algorithm*}[tpb]
\caption{Precursor miRNA prediction}\label{alg:pseudo}
\begin{multicols}{2}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} $x_s=\langle x_{s,1},x_{s,2},\ldots,x_{s,|x_s|} \rangle$ where $x_s \in X_s$, $y$ 
\LCOMMENT{$X$: A set of sequences. $|X_s|=N$}
\LCOMMENT{$x_s$: A precursor miRNA sequence with its length of $|x_s|$ and $x_{s,i}\in\{A,C,G,U\}$ for $i=1,2,\ldots,|x_s|$}
\LCOMMENT{$y$: A true label for $x_s$. $y \in\{0,1\}$}
\STATE {\bfseries Param:} $m$: mini-batch size
\STATE {\bfseries Output:} $W = \{w_e,w_l,w_f\}$
\LCOMMENT{$W$: Whole model weights composed of weights of embedding layers ($w_e$), LSTM layers ($w_l$), fully connected layers ($w_f$)}

\LCOMMENTR{\bfseries Step 1: Preprocessing~(Section~\ref{preprocessing})}
\NoDo\FOR{each sequence in $X_s$}
\STATE $x_t \gets \text{fold}(x_s)$
\LCOMMENT{fold: A function to predict a secondary structure of a given sequence $x_s$}
\LCOMMENT{$x_t$: A dot-bracket notated secondary structure of given input sequence $x_s$. $|x_t|=|x_s|$ and $x_t=\langle x_{t,1},x_{t,2},\ldots,x_{t,|x_t|}$ where $x_{t,i}\in\{(,.,)\}$ for $i=1,2,\ldots,|x_t|$}
\STATE $(x_f,x_b) \gets \text{split}(x_t)$
\LCOMMENT{split: A function to split a given secondary structure $x_s$ into a forward structure $x_f$ and a backward structure $x_b$}
\LCOMMENT{$x_f=\langle x_{t,1},x_{t,2},\ldots,x_{t,k-1}\rangle$ and $x_b=\langle x_{t,k},x_{t,k+1},\ldots,x_{t,|x_t|}\rangle$ for pre-determined position $k$}
\STATE $x_r \gets \text{flip}(x_b)$
\LCOMMENT{flip: A function to flip a given structure $x_b$}
\LCOMMENT{$x_r$: The flipped structure of $x_b$. $x_r=\langle x_{t,|x_t|},x_{t,{|x_t|-1}},\ldots,x_{t,k}\rangle$}
\ENDFOR
\LCOMMENTR{The outputs of preprocessing are grouped into $X_f$ and $X_r$ where $x_f \in X_f$ and $x_r \in X_r$ respectively}

\LCOMMENTR{\bfseries Step 2: Training on neural network~(Section~\ref{nnlayer})}
\STATE initializing weights $W$
\NoDo\FOR{each epoch}
\NoDo\FOR{$m$ training data of $x_s$, $x_f$ and $x_r$ randomly picked from dataset $X_s$,$X_f$, and $X_r$}

\LCOMMENTR{\bfseries Embedding Layers}
\STATE $x_{s}'\gets \text{embed}_\text{seq}(x_s)$
\STATE $x_{f}'\gets \text{embed}_\text{f-str}(x_f)$
\STATE $x_{r}'\gets \text{embed}_\text{b-str}(x_r)$
\LCOMMENT{embed: Embedding layer to return a matrix for an input tuple}
\LCOMMENT{$x_{s}'$ is $\sss |x_s| \times 4$ matrix. $x_{f}'$ and $x_{r}'$ are the matrices of $\sss |x_f| \times 3$ and $\sss |x_r| \times 3$, respectively}

\LCOMMENTR{}
\LCOMMENTR{\bfseries LSTM Layers}
\STATE $h_s \gets \text{LSTM}_\text{seq}(x_{s}')$
\STATE $h_f \gets \text{LSTM}_\text{f-str}(x_{f}')$
\STATE $h_r \gets \text{LSTM}_\text{b-str}(x_{r}')$
\LCOMMENT{LSTM: LSTM layer to return a vector for an input matrix}
\LCOMMENT{$h_s$,$h_f$, and $h_r$ are 10-dim vectors for the output of each LSTM layer.}

\LCOMMENTR{}
\LCOMMENTR{\bfseries Fully Connected Layers}
\STATE $y_s \gets \text{fcl}_\text{seq}(h_s)$
\STATE $y_t \gets \text{fcl}_\text{str}({h_f}^\frown h_r)$
\LCOMMENT{fcl: Fully connected layer to return an output vector}
\LCOMMENT{$\text{fcl}_\text{seq}$: 10-dim input and 2-dim output}
\LCOMMENT{$\text{fcl}_\text{str}$: 20-dim input and 2-dim output}
\LCOMMENT{$^\frown$: vector concatenate operation}
\STATE $\hat{y} \gets \text{fcl}_\text{multi}({y_s}^\frown y_t)$
\LCOMMENT{$\text{fcl}_\text{multi}$: 4-dim input and 2-dim output}
\ENDFOR


%%% on doing!!
\LCOMMENTR{}
\LCOMMENTR{\bfseries Weights Updating}
\STATE $E \gets -\frac{1}{m} \sum_{m} (\hat{y}-y)^2$
\LCOMMENT{E: Mini-batch training error using mean squared error}
\STATE $W \gets W - \bigtriangleup W$
\LCOMMENT{Calculating $\bigtriangleup W$ based on $E$ using gradient descent optimization algorithm ``Adam''}
\ENDFOR
\end{algorithmic}
\end{multicols}
\end{algorithm*}

